Neural Transductive Learning and Beyond: Morphological Generation in the Minimal-Resource Setting

Neural state-of-the-art sequence-to-sequence (seq2seq) models often do not perform well for small training sets. We address paradigm completion, the morphological task of, given a partial paradigm, generating all missing forms. We propose two new methods for the minimal-resource setting: (i) Paradigm transduction: Since we assume only few paradigms available for training, neural seq2seq models are able to capture relationships between paradigm cells, but are tied to the idiosyncracies of the training set. Paradigm transduction mitigates this problem by exploiting the input subset of inflected forms at test time. (ii) Source selection with high precision (SHIP): Multi-source models which learn to automatically select one or multiple sources to predict a target inflection do not perform well in the minimal-resource setting. SHIP is an alternative to identify a reliable source if training data is limited. On a 52-language benchmark dataset, we outperform the previous state of the art by up to 9.71% absolute accuracy.

==> results_table.tex <==
1 & albanian & .0385
%& .0000 
& .0305 & .1224 & .2742 & \textbf{.6793} & .6568 & .0385 & .0055 & .0305 & .8362 & .2335 & .8786 & \textbf{.8891} & .0385 & .1808 & .0305 & .8951 & .4276 & \textbf{.9750} & .9700 \\
2 & arabic & .0334
%& .0000 
& .0445 & .4262 & .4744 & \textbf{.8191} & .8006 & .0334 & .0378 & .0445 & .5389 & .7265 & .8962 & \textbf{.9096} & .0334 & .3988 & .0445 & .5567 & .7509 & .9400 & \textbf{.9526} \\
3 & armenian & .0233
%& .0000 
& .0841 & .7912 & .9002 & \textbf{.9235} & .9174 & .0233 & .0319 & .0841 & .8089 & .9706 & .9762 & \textbf{.9787} & .0233 & .5297 & .0841 & .8611 & .8049 & \textbf{.9919} & .9899 \\
4 & bulgarian & .0854
%& .0000 
& .0151 & .3920 & \textbf{.4958} & .4807 & .4774 & .0854 & .0318 & .0151 & .4908 & \textbf{.5444} & .5243 & .5427 & .0854 & .2663 & .0151 & .7471 & \textbf{.8425} & .8208 & .8191 \\
5 & catalan & .0173
%& .0000 
& .0210 & \textbf{.9407} & .9346 & .8758 & .8655 & .0173 & .0415 & .0210 & .9533 & \textbf{.9706} & .9659 & .9641 & .0173 & .5626 & .0210 & .9603 & .9795 & \textbf{.9897} & .9874 \\
6 & czech & .1255
%& .0000 
& .0498 & .2656 & \textbf{.3503} & .2873 & .3122 & .1255 & .0166 & .0498 & .5643 & \textbf{.5873} & .5332 & .5373 & .1255 & .2739 & .0498 & .8579 & \textbf{.8794} & .8444 & .8423 \\
7 & danish & .1738
%& .0000 
& .0230 & \textbf{.4230} & \textbf{.4230} & .1705 & .1738 & .1738 & .0492 & .0230 & \textbf{.7016} & \textbf{.7016} & .4918 & .5016 & .1738 & .4984 & .0230 & \textbf{.7574} & .7541 & .3541 & .4066 \\
8 & dutch & .1661
%& .0000 
& .0018 & .4963 & \textbf{.5664} & .4908 & .4982 & .1661 & .0424 & .0018 & .6771 & \textbf{.8653} & .7841 & .7915 & .1661 & .4317 & .0018 & .7804 & \textbf{.8856} & .8727 & .8727 \\
9 & english & .2080
%& .0000 
& .0240 & \textbf{.7640} & \textbf{.7640} & .4000 & .4000 & .2080 & .0600 & .0240 & \textbf{.8400} & \textbf{.8400} & .7360 & .7360 & .2080 & .6680 & .0240 & \textbf{.9120} & \textbf{.9120} & .8440 & .8440 \\
10 & faroese & .1570
%& .0000 
& .0239 & .4978 & \textbf{.5755} & .3991 & .3946 & .1570 & .0149 & .0239 & .5919 & \textbf{.6831} & .6069 & .6024 & .1570 & .3602 & .0239 & .7010 & \textbf{.7549} & .7175 & .7160 \\
11 & finnish & .0650
%& .0000 
& .0257 & .6082 & \textbf{.7630} & .6330 & .6236 & .0650 & .0274 & .0257 & .6279 & \textbf{.8896} & .8777 & .8760 & .0650 & .3311 & .0257 & .6929 & .9264 & \textbf{.9615} & .9504 \\
12 & french & .0213
%& .0000 
& .0142 & .8709 & \textbf{.9040} & .8918 & .8943 & .0213 & .0930 & .0142 & .8516 & .9233 & .9487 & \textbf{.9517} & .0213 & .6880 & .0142 & .9263 & .9548 & .9964 & \textbf{.9980} \\
13 & georgian & .0534
%& .0000 
& .0036 & .7886 & \textbf{.8682} & .7684 & .7613 & .0534 & .1235 & .0036 & .8242 & \textbf{.8967} & .8753 & .8646 & .0534 & .6211 & .0036 & .9097 & \textbf{.9549} & .9335 & .9477 \\
14 & german & .2959
%& .0000 
& .0174 & .6983 & \textbf{.7466} & .6460 & .6267 & .2959 & .0000 
& .0174 & .7041 & \textbf{.8375} & .7485 & .7563 & .2959 & .4391 & .0174 & .7640 & .8549 & \textbf{.8743} & \textbf{.8743} \\
15 & hebrew & .0507
%& .0000 
& .0178 & .3238 & .6148 & \textbf{.6548} & .6459 & .0507 & .2109 & .0178 & .4270 & .6530 & \textbf{.8639} & .8585 & .0507 & .5329 & .0178 & .5427 & .6984 & .9137 & \textbf{.9377} \\
16 & hindi & .0038
%& .0000 
& .6005 & .6449 & .7082 & \textbf{.9405} & .9264 & .0038 & .0000 
& .6005 & .7031 & .8565 & \textbf{.9504} & .9496 & .0038 & .3621 & .6005 & .9539 & .4922 & .9979 & \textbf{1.000} \\
17 & hungarian & .0310
%& .0000 
& .0038 & .1791 & \textbf{.5489} & .5435 & .5488 & .0310 & .0060 & .0038 & .4452 & \textbf{.7621} & .7498 & .7415 & .0310 & .3447 & .0038 & .5412 & .8237 & .9108 & \textbf{.9146} \\
18 & icelandic & .1640
%& .0000 
& .0148 & .4579 & \textbf{.5657} & .4106 & .4136 & .1640 & .0295 & .0148 & .5451 & \textbf{.6721} & .4993 & .5288 & .1640 & .2393 & .0148 & .6691 & .7474 & \textbf{.7696} & .7430 \\
19 & italian & .0186
%& .0000 
& .0100 & .6643 & \textbf{.7200} & .6962 & .6976 & .0186 & .0190 & .0100 & .7186 & .7767 & .9052 & \textbf{.9233} & .0186 & .3171 & .0100 & .7305 & .7848 & \textbf{.9733} & .9719 \\
20 & latvian & .0735
%& .0000 
& .0115 & .6888 & \textbf{.7579} & .4971 & .5115 & .0735 & .0101 & .0115 & .7983 & \textbf{.8919} & .7752 & .7680 & .0735 & .5086 & .0115 & .8646 & \textbf{.9669} & .9179 & .9150 \\
21 & sorbian & .0799
%& .0000 
& .0237 & .3758 & .5643 & .5793 & \textbf{.6080} & .0799 & .1024 & .0237 & .6592 & \textbf{.8402} & .7328 & .7553 & .0799 & .5031 & .0237 & .8227 & \textbf{.8901} & .8664 & .8739 \\
22 & maced. & .0959
%& .0000 
& .0072 & .4249 & \textbf{.6023} & .4149 & .4077 & .0959 & .0615 & .0072 & .8655 & \textbf{.8898} & .7611 & .7954 & .0959 & .5722 & .0072 & .8970 & \textbf{.9714} & .9614 & .9599 \\
23 & navajo & .0589
%& .0123 
& .0014 & .2658 & \textbf{.3563} & .0466 & .0370 & .0589 &
.0616 & .0014 & .3315 & \textbf{.4801} & .0329 & .0315 &
.0589 & .2849 & .0014 & .3795 & \textbf{.5695} & .0301 &
.0137 \\
24 & sami & .0436
%& .0000 
& .0048 & .1562 & \textbf{.3986} & .2890 & .3046 & .0436 & .0155 & .0048 & .3172 & \textbf{.8351} & .7856 & .7818 & .0436 & .2250 & .0048 & .4568 & .9108 & .9108 & \textbf{.9176} \\
25 & nynorsk & .1043
%& .0000 
& .0245 & \textbf{.4233} & \textbf{.4233} & .1043 & .1043 & .1043 & .0123 & .0245 & \textbf{.6074} & \textbf{.6074} & .3067 & .3129 & .1043 & .4785 & .0245 & .6442 & \textbf{.6626} & .4172 & .4294 \\
26 & persian & .0218
%& .0000 
& .2400 & .7342 & .1633 & \textbf{.9880} & .9844 & .0218 & .0509 & .2400 & .7829 & .1815 & .9898 & \textbf{.9960} & .0218 & .6073 & .2400 & .7644 & .1971 & \textbf{.9993} & .9989 \\
27 & polish & .0986
%& .0000 
& .0218 & .5672 & \textbf{.6453} & .5928 & .5826 & .0986 & .0205 & .0218 & .8028 & \textbf{.8271} & .7631 & .7452 & .0986 & .3995 & .0218 & \textbf{.9001} & .8924 & .8515 & .8553 \\
28 & portug. & .0697
%& .0000 
& .0432 & .9171 & \textbf{.9694} & .9135 & .9190 & .0697 & .1058 & .0432 & .9529 & \textbf{.9858} & .9784 & .9742 & .0697 & .6829 & .0432 & .9616 & \textbf{.9861} & .9839 & .9823 \\
29 & quechua & .0083
%& .0000 
& .5093 & .9133 & \textbf{.9998} & .9835 & .9856 & .0083 & .2750 & .5093 & .9134 & \textbf{.9999} & .9887 & .9926 & .0083 & .7852 & .5093 & .8913 & \textbf{.9994} & .9965 & \textbf{.9994} \\
30 & russian & .1166
%& .0000 
& .0092 & .4018 & \textbf{.4617} & .3221 & .3528 & .1166 & .0598 & .0092 & .8298 & \textbf{.8574} & .7715 & .7761 & .1166 & .6610 & .0092 & .8589 & \textbf{.8712} & .8635 & .8650 \\
31 & gaelic & .3684
%& .0000 
& .0202 & .4413 & \textbf{.5061} & .4170 & .3927 &.3684
& .0000 
& .0202 & .4130 & \textbf{.4858} & .4413 & .4575 & - & - & - & - & - & - & - \\
32 & SCB & .0870
%& .0000 
& .2802 & .3007 & .3116 & \textbf{.5266} & .5133 &.0870
& .0000 
& .2802 & .3684 & .3744 & \textbf{.6401} & .6196 & .0870 & .0918 & .2802 & .8575 & .7536 & .8829 & \textbf{.8841} \\
33 & slovak & .1301
%& .0000 
& .0053 & .4439 & \textbf{.5365} & .3226 & .3012 & .1301 & .0160 & .0053 & .5936 & \textbf{.6667} & .4011 & .3993 & .1301 & .3119 & .0053 & .6934 & \textbf{.7184} & .6310 & .6275 \\
34 & slovene & .1094
%& .0000 
& .0151 & .5774 & \textbf{.7928} & .5925 & .5867 & .1094 & .0012 & .0151 & .6787 & .8510 & .8254 & \textbf{.8661} & .1094 & .4505 & .0151 & .7648 & .9302 & \textbf{.9430} & .9336 \\
35 & spanish & .0144
%& .0000 
& .0207 & .8067 & .8835 & \textbf{.9186} & .9088 & .0144 & .0330 & .0207 & .9218 & .8884 & \textbf{.9768} & .9709 & .0144 & .5884 & .0207 & .9358 & .8891 & .9853 & \textbf{.9874} \\
36 & swedish & .1824
%& .0000 
& .0441 & .4353 & \textbf{.5118} & .2735 & .2735 & .1824 & .0441 & .0441 & .5735 & \textbf{.7088} & .5176 & .5265 & .1824 & .4206 & .0441 & .7824 & \textbf{.8471} & .7235 & .7353 \\
37 & turkish & .0168
%& .0000 
& .0894 & .2050 & .6984 & \textbf{.8748} & .8643 & .0168 & .0358 & .0894 & .7204 & .9258 & \textbf{.9754} & .9740 & .0168 & .5388 & .0894 & .8673 & .9402 & .9934 & \textbf{.9941} \\
38 & ukrainian & .0873
%& .0000 
& .0159 & .4222 & \textbf{.4921} & .3460 & .3206 & .0873 & .0413 & .0159 & \textbf{.6714} & .6619 & .5857 & .5984 & .0873 & .3984 & .0159 & .7397 & \textbf{.7619} & .7413 & .7508 \\
39 & urdu & .0264
%& .0000 
& .5434 & .8059 & .8059 & \textbf{.8754} & .8720 & .0264 & .0014 & .5434 & .8102 & .8102 & .9438 & \textbf{.9485} & .0264 & .2007 & .5434 & .9533 & .7040 & .9887 & \textbf{.9901} \\
40 & welsh & .0277
%& .0000 
& .0147 & .5167 & .4319 & .9104 & \textbf{.9128} & .0277 & .0513 & .0147 & .8280 & .8843 & .9707 & \textbf{.9756} & .0277 & .3504 & .0147 & .8525 & .9446 & .9886 & \textbf{.9919} \\\hline
41 & basque
& .0004
%& .0000
& .6743 & .0050 & .1034 & .9298 & \textbf{.9427}
& .0004 
& .0108 & .6743 & .0457 & .0968 & .9132 & \textbf{.9190} & - & - & - & - & - & - & - \\
42 & bengali & .0357
%& .0000 
& .0127 & .7720 & \textbf{.9019} & .6675 & .6599 & .0357 & .0102 & .0127 & .8586 & \textbf{.9172} & .8344 & .8089 & .0357 & .0701 & .0127 & .8752 & \textbf{.9248} & .8675 & .8713 \\
43 & estonian & .0373
%& .0006 
& .0210 & .3888 & .6857 & .7881 & \textbf{.7992} & .0373 & .0081 & .0210 & .6257 & .7119 & \textbf{.9173} & \textbf{.9173} & .0373 & .2893 & .0210 & .7730 & .7189 & .9761 & \textbf{.9796} \\
44 & haida & .0087
%& .0000 
& .0981 & .4715 & .9452 & .9279 & \textbf{.9611} &
.0087
& .0000 
& .0981 & .6453 & .9481 & .9394 & \textbf{.9762} & - & - & - & - & - & - & - \\
45 & irish & .1971
%& .0000 
& .0128 & .3230 & \textbf{.4343} & .3248 & .3285 & .1971 & .0109 & .0128 & .4033 & .4872 & .5675 & \textbf{.5766} & .1971 & .2518 & .0128 & .4799 & .5712 & \textbf{.6788} & .6588 \\
46 & khaling
%& .0007 
& .0209 & .5773 & .4230 & .4422 & .9686
& \textbf{.9716}
& .0007 
& .2258 & .5773 & .5820 & .6208 & \textbf{.9918} &
.9895
& .0007 
& .6979 & .5773 & .7908 & .6583 & .9960 & \textbf{.9983} \\
47 & kurmanji & .0817
%& .0000 
& .0174 & .7843 & \textbf{.8017} & .4591 & .4539 & .0817 & .0765 & .0174 & .8835 & \textbf{.8887} & .7965 & .8330 & .0817 & .7165 & .0174 & \textbf{.9287} & .9165 & \textbf{.9287} & .9183 \\
48 & latin & .0600
%& .0000 
& .0146 & .2416 & \textbf{.5198} & .3016 & .2899 &
.0600
& .0000 
& .0146 & .3909 & \textbf{.8507} & .4905 & .5168 & .0600 & .2050 & .0146 & .4671 & \textbf{.8814} & .6852 & .7379 \\
49 & lithuanian & .0169
%& .0000 
& .0125 & .3845 & \textbf{.4951} & .4790 & .4835 & .0169 & .0134 & .0125 & .6619 & \textbf{.8287} & .7395 & .7431 & .0169 & .2810 & .0125 & .6048 & \textbf{.8582} & .8260 & .8359 \\
50 & bookmal & .1321
%& .0000 
& .0377 & .4025 & \textbf{.4151} & .1069 & .1069 & .1321 & .0377 & .0377 & \textbf{.5094} & \textbf{.5094} & .3585 & .3585 & .1321 & .4277 & .0377 & .6792 & \textbf{.6855} & .5094 & .5157 \\
51 & romanian & .0754
%& .0000 
& .0133 & .1420 & \textbf{.2500} & .1317 & .1213 & .0754 & .0074 & .0133 & .6154 & \textbf{.7663} & .5814 & .6124 & .0754 & .2914 & .0133 & \textbf{.7988} & .7825 & .7500 & .7544 \\
52 & sorani & .0110
%& .0000 
& .1285 & .5478 & .5435 & .6162 & \textbf{.6272} & .0110 & .0042 & .1285 & .6839 & .5773 & .8216 & \textbf{.8225} & .0110 & .2984 & .1285 & .7210 & .6044 & .8512 & \textbf{.8529} \\\hline
53 & {\bf average} & .0810
%& .0006 
& .0883 & .5012 & \textbf{.5971} & .5808 & .5793 & .0810 & .0432 & .0883 & .6576 & .7355 & .7486 & \textbf{.7547} & .0782 & .4211 & .0775 & .7707 & .8008 & .8454 & \textbf{.8483} 

